A Framework for Ethical Judgment of Smart City Applications

As modern cities increasingly adopt a variety of sensors and Internet of Things (IoT) technologies to collect and analyze data about residents, environments, and public services, they are fostering greater interactions among smart city applications, residents, governments, and businesses. This trend makes it essential for regulators to focus on these interactions to manage smart city practices effectively and prevent unethical outcomes. To facilitate ethical analysis for smart city applications, this paper introduces a judgment framework that examines various scenarios where ethical issues may arise. Employing a multi-agent approach, the framework incorporates diverse social entities and applies logic-based ethical rules to identify potential violations. Through a rights-based analysis, we developed a set of 13 ethical principles and rules to guide ethical practices in smart cities. We utilized two specification languages, Prototype Verification System (PVS) and Alloy, to model our multi-agent system. Our analysis suggests that Alloy may be more efficient for formalizing smart cities and conducting ethical rule checks, particularly with the assistance of a human evaluator. Simulations of a real-world smart city application demonstrate that our ethical judgment framework effectively detects unethical outcomes and can be extended for practical use.

==> figures/table-compare-mmi.tex <==
\begin{table*}[t]
\caption{Performance Comparison - MMI\tnote{1}}
\begin{center}
\begin{threeparttable}
\begin{tabular}{c r r r r r r r}
    \hline\hline
    \textbf{Model} & \textbf{BLEU} & \textbf{ROUGE1-Precision} & \textbf{ROUGE1-Recall} & \textbf{ROUGE1-F1} & \textbf{ROUGE1-Precision} & \textbf{ROUGE1-Recall} & \textbf{ROUGE1-F1} \\ 
    \hline
    Seq2Seq        &  0.090 &  0.225 &	0.077 & 0.080 &	0.013 & 0.003 & 0.004 \\
    Proposed       &  \textbf{0.132} &  0.153 &	\textbf{0.148} &	0.097 &	0.025 &	0.018 &	0.015 \\
    Seq2Seq + MMI  &  0.104 &  0.268 &	0.112 &	0.109 & 0.030 & 0.007 & 0.011 \\
    Proposed + MMI &  0.111 &  \textbf{0.300} &	0.112 &	\textbf{0.127} & \textbf{0.052} & \textbf{0.022} & \textbf{0.028} \\
    \hline
\end{tabular}
\begin{tablenotes}
\item[1] This table is only for illustration purpose. The models are not fully trained. 
\end{tablenotes}
\end{threeparttable}
\end{center}
\label{tbl:compare}
\end{table*}
